The Reversal Ratio of a Poset

Felsner and Reuter introduced the linear extension diameter of a partially ordered set $\mathbf{P}$, denoted $\mbox{led}(\mathbf{P})$, as the maximum distance between two linear extensions of $\mathbf{P}$, where distance is defined to be the number of incomparable pairs appearing in opposite orders (reversed) in the linear extensions. In this paper, we introduce the reversal ratio $RR(\mathbf{P})$ of $\mathbf{P}$ as the ratio of the linear extension diameter to the number of (unordered) incomparable pairs. We use probabilistic techniques to provide a family of posets $\mathbf{P}_k$ on at most $k\log k$ elements for which the reversal ratio $RR(\mathbf{P}_k)\leq C/\log k$, where $C$ is a constant. We also examine the questions of bounding the reversal ratio in terms of order dimension and width.

==> mitch.tex <==
\usepackage{amsmath, amsthm, amssymb, amsfonts}
%\usepackage[mathscr]{eucal}
\usepackage{mathrsfs}

\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\lcm}{lcm}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\rad}{rad}
\DeclareMathOperator{\intr}{Int}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\Gal}{Gal}
                                %       Theorem environments

%% \theoremstyle{plain} %% This is the default
\newtheorem{thm}{Theorem}%[section]
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{ax}{Axiom}
\newtheorem*{thm*}{Theorem}
\newtheorem*{cor*}{Corollary}
\newtheorem*{lem*}{Lemma}
\newtheorem*{prop*}{Proposition}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem*{defn*}{Definition}
\newtheorem{ex}{Exercise}
\newtheorem{hw}{Homework}
\newtheorem{prob}{Problem}
\newtheorem*{prob*}{Problem}

\theoremstyle{definition}
\newtheorem{rem}[thm]{Remark}

\theoremstyle{definition}
\newtheorem{conj}{Conjecture}
\newtheorem*{conj*}{Conjecture}
\newtheorem{claim}[thm]{Claim}
\newtheorem{examp}[thm]{Example}
\newtheorem*{example*}{Example}
%\newtheorem{question}{Question}

\newtheorem*{notation}{Notation}

                                %\numberwithin{equation}{section}

\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\propref}[1]{Proposition~\ref{#1}}
%\newcommand{\corref}[1]{Corollary~\ref{#1}}
%\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\remref}[1]{Remark~\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\figref}[1]{Figure~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}

                                %Math Definitions

\newcommand{\Hom}[3]{\text{Hom}_{#1}(#2,#3)}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\mscr}[1]{\mathscr{#1}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mfr}[1]{\mathfrak{#1}}
\newcommand{\mr}[1]{\mathrm{#1}}


\newcommand{\Q}{{\mathbb Q}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\C}{{\mathbb C}}
\newcommand{\N}{{\mathbb N}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\T}{{\mathbb T}}
\newcommand{\D}{{\mathbb D}}
\renewcommand{\P}{{\mathbb P}}
%\newcommand{\presentation}[2]{\ensuremath{\langle #1 \mid #2 \rangle}}
\newcommand{\sprod}[2]{\left\langle #1,#2\right\rangle}
%\renewcommand{\theenumi}{\alph{enumi}}
%\renewcommand{\theenumii}{\arabic{enumii}}
\newcommand{\Neq}[1]{\mathbf{N}_{=}(\{#1\})}
\newcommand{\Ngeq}[1]{\mathbf{N}_{\geq}(\{#1\})}
\newcommand{\inv}{\ensuremath{^{-1}}}
\newcommand{\normal}{\vartriangleleft}
\newcommand{\nin}{\not\in}
\newcommand{\esprod}{\sprod{\,}{\,}}
\DeclareMathOperator{\diag}{diag}
%\newcommand{\Hom}[3]{{\mathrm{Hom}_{#1} (#2 , \, #3)}}
%\newcommand{\sprod}[2]{\langle #1,#2\rangle}
%\newcommand{\rad}[1]{\text{\rm{Rad}}\esprod_{#1}}
\DeclareMathOperator{\Rad}{Rad}
\newcommand{\empset}{\{\}}
\renewcommand{\today}{\number \day \space \ifcase \month \or January\or%
  February\or March\or April\or May\or June\or July\or August\or%
  September\or October\or November\or December\fi \space \number \year}
\newcommand{\bs}{\backslash}
\newcommand{\meet}{\wedge}
\newcommand{\join}{\vee}

\newcommand{\covered}{\lessdot}
\newcommand{\covers}{\gtrdot}
\DeclareMathOperator{\ld}{ld}
\DeclareMathOperator{\weakd}{wd}
\DeclareMathOperator{\width}{width}
\DeclareMathOperator{\inc}{inc}
\DeclareMathOperator{\Inc}{Inc}
\DeclareMathOperator{\height}{height}
\DeclareMathOperator{\sdepth}{sdepth}
\DeclareMathOperator{\depth}{depth}
\DeclareMathOperator{\led}{led}
\DeclareMathOperator{\dist}{dist}


\newcommand{\abs}[1]{\ensuremath{\left| #1 \right|}}
\DeclareMathOperator{\bw}{bw}
%\DeclareMathOperator{\bandwidth}{bw}
%\newcommand{\bw}[1]{\ensuremath{\bandwidth\!\left(#1\right)}}
\newcommand{\incomp}[1][{}]{\!\ensuremath{\parallel_{#1}}\!}
\newcommand{\maxdeg}[1]{\ensuremath{\Delta\!\left(#1\right)}}
\newcommand{\maxinc}[1]{\maxdeg{#1}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor #1 \right\rfloor}}
\newcommand{\ceil}[1]{\ensuremath{\left\lceil #1 \right\rceil}}
\newcommand{\order}[1]{\ensuremath{\left| #1 \right|}}
\newcommand{\ileft}[2][{}]{\ensuremath{\ell_{#1}(#2)}}
\newcommand{\iright}[2][{}]{\ensuremath{\mathit{r}_{#1}(#2)}}
\newcommand{\up}[1]{\ensuremath{U(#1)}}
\newcommand{\down}[1]{\ensuremath{D(#1)}}
\DeclareMathOperator{\critical}{crit}
\newcommand{\crit}[1]{\ensuremath{\critical\left(#1\right)}}
\newcommand{\PXP}{\mbf{P}=(X,\leq_P)}
